Octopus: A Fair Packet Delivery Service

The packet delivery fairness is critical in many applications in the cloud, such as exchange systems, consensus protocols, and online gaming applications. However, due to nonidentical and dynamic packet forwarding paths, as well as many in-network queuing delays, supporting packet delivery fairness is challenging in a shared compute environment. In this paper, we present Octopus, the first general fair packet delivery service to achieve packet arrival time variations smaller than tens of nanoseconds, with the existence of latency variations in the network. The key ideas of Octopus to support such good fairness come from repurposing hardware traffic shaping capabilities in modern NICs, and deploying agents at local SmartNICs to minimize latency variations from packet forwarding. Evaluation results show that Octopus has less than 40 ns unfairness for up to 99.97\% multicast packets.

==> implementation.tex <==
\section{Implementation}
\yl{I don't think this section is necessary}

\noindent\textbf{\sys{} packet format.}
\sys{} uses the gRPC protocol \yl{Do you mean protobuf, or gRPC?} to encode the intended packet releasing time into the packet.
To guarantee the releasing time is recognized correctly by all agents, the clocks on the sender and agents are well synchronized.

\noindent\textbf{\sys{} sender interface.}
\sys{} sender interface is written in a user-space library with around 700 lines of C/C++ codes.
The sender interface uses a user-space packet I/O library to achieve better performance.
Upon receiving a message from the sender application, it first determines the intended releasing time for all agents.
Such releasing time is calculated by adding a specific delay on the current timestamp, and the delay is determined by the upper bound of the packet forwarding latency and the packet I/O call latency.

\noindent\textbf{\sys{} agent.}
\sys{} agent is written in a user-space program with around 1000 lines of C/C++ codes.
The agent uses a user-space packet I/O library to achieve better performance.
To be specific, the agent receives incoming packets in poll mode to minimize software delays.
The agent runs on the independent Linux system of the SmartNIC.

==> overview.tex <==
\section{Overview}
\label{sec:overview}

\subsection{System Architecture}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{architecture.png}
    \caption{The architecture of Octopus. Note that grey boxes (the sender application and receiver applications) are not part of the architecture.}
    \label{fig:architecture}
\end{figure}

Figure \ref{fig:architecture} shows a high-level architecture of \sys{}.
\sys{} consists of the following components: a market engine, a set of market participants, and a set of agents.
The market engine and market participants can be at any location in the network, while the agent runs on the SmartNIC associated with the corresponding market participant server or the market engine server.

\mypara{Global clock synchronization}
\sys{} first deploys a global clock synchronization service for the sender's server and all agents.
This synchronization service helps the sender and agents to agree on a same packet delivery time globally.


\mypara{\sys{} agents}
Agents are responsible to control the packet release time towards receiver applications.
For each receiver application, one agent is deployed on the local SmartNIC associated with the same server running the receiver, and it receives all incoming packets from the sender on behalf of the corresponding receiver.
Upon receiving each packet, the agent parses the intended release time provided by the sender (see below), and releases the packet on the intended time.

\mypara{\sys{} sender interface}
The sender interface is called by the sender application (\textit{e.g., } the market engine in exchange systems) to start a fair packet delivery service.
For each packet to be multicasted from the sender, the sender interface is responsible to determine a same intended release time for all agents, and tags the timestamp along with the packet.

\mypara{Packet delivery steps}
\sys{} multicasts a packet in the following steps.
\begin{enumerate}
    \item The sender application generates a packet to multicast to all receiver applications, and calls the \sys{} sender interface to help multicast the packet.
    \item The \sys{} sender interface determines a global release time (which is calculated as the current timestamp plus a predefined delay $\delta$), and tags the timestamp along with the packet.
    \item The interface sends the tagged packet to all agents.
    \item The agents receive the tagged packet, parse the release time, hold the packet, and release the packet to its corresponding receiver application at the release time.
\end{enumerate}

\subsection{Key Ideas}

\sys{} has the following two key ideas to achieve good fairness for the market system.

\begin{enumerate}
    \item \textbf{Time based packet releasing feature.} Many modern NICs support hardware traffic shaping feature to control packet sending rate, which allows users to specify an intended release time for each packet. This feature allows \sys{} to deploy an agent close to each receiver, and let the agent to control the packet delivery time towards the receiver. 
    \item \textbf{Deploying agents at local SmartNICs.} \sys{} decides to deploy the agent at local SmartNICs of the server running the receiver. 
    Since the local SmartNIC is close to the receiver on the same server, the packet forwarding delay variance is minimized between the agent and the receiver.
\end{enumerate}
